Exact and Efficient Parallel Inference for Nonparametric Mixture Models

Nonparametric mixture models based on the Dirichlet process are an elegant alternative to finite models when the number of underlying components is unknown, but inference in such models can be slow. Existing attempts to parallelize inference in such models have relied on introducing approximations, which can lead to inaccuracies in the posterior estimate. In this paper, we describe auxiliary variable representations for the Dirichlet process and the hierarchical Dirichlet process that allow us to sample from the true posterior in a distributed manner. We show that our approach allows scalable inference without the deterioration in estimate quality that accompanies existing methods.

==> related.tex <==
\section{Related Work}\label{sec:related}
A number of inference schemes have been developed for the DP and the HDP. The most commonly used class of inference methods is based on the Chinese restaurant process (CRP, see for example \cite{Aldous:1983}). Such schemes integrate out the random measures ($D$ in Eq.~\ref{eq:DP}; $D_0$ and $\{D_m\}_{m=1}^M$ in Eq.~\ref{eq:HDP}) to obtain the conditional distribution for the cluster allocation of a single data point, conditioned on the allocations of all the other data points. A variety of Gibbs samplers based on the CRP can be constructed for the DP \cite{Neal:1998} and the HDP \cite{Teh:Jordan:Beal:Blei:2006}.
Unfortunately, because the conditional distribution for the cluster allocation of a single data point depends on all the data, this step cannot be parallelized without introducing approximations.

An alternative class of inference schemes involve explicitly instantiating the random measures \cite{Ishwaran:James:2001}. In this case, the observations are i.i.d. given the random measures, and can be sampled in parallel. However, since the random measure depends on the cluster allocations of all the data points, sampling the random measure cannot be parallelized.

Among existing practical schemes for parallelizable inference in DP and HDP, the following three are the most popular:
% Sequential sampling schemes; mean field inference in a variational approximation; and approximating the conditional distributions in a CRP-based Gibbs sampler.

\subsection{Sequential Monte Carlo methods}
Sequential Monte Carlo (SMC) methods approximate a distribution of interest using a swarm of weighted, sequentially updated, particles. SMC methods have been used to perform inference in a number of models based on the DP \cite{Fearnhead:2004,Ulker:Gunsel:Cemgil:2010,Rodriguez:2011,Ahmed:Ho:Teo:Eisenstein:Smola:Xing:2011}. Such methods are appealing when considering parallelization, because each particle (and its weight) are updated independently of the other particles, and need consider only one data point at a time. However, a naive implementation where each particle is propagated in isolation leads to very high variance in the resulting estimate. To avoid this, it is typical to introduce \emph{resampling} steps, where the current swarm of particles is replaced by a new swarm sampled from the current posterior estimate. This avoids an explosion in the variance of our estimate, but the resampling cannot be performed in parallel. %Another problem often encountered in SMC models is particle degeneracy -- resampling steps mean that our estimate can consist of very few unique particle paths, especially in describing the first observations. A standard method to resolve this problem is to add ``jitter'' to the particles using MCMC steps. However, these MCMC steps are not easily parallelizable.

\subsection{Variational inference}
Variational Bayesian inference algorithms have been developed for both the DP \cite{Blei:Jordan:2004, Kurihara:Welling:Teh:2007} and the HDP \cite{Teh:Kurihari:Welling:2007, Wang:Paisley:Blei:2011}. Variational methods approximate a posterior distribution $p(\theta|X)$ with a distribution $q(\theta)$ belonging to a more manageable family of distributions and try to find the ``best'' member of this family, typically by minimizing the Kullback-Leibler divergence between $p(\theta|X)$ and $q(\theta)$. This also gives us a lower bound on the log likelihood, $\log p(X)$. A typical approach to selecting the family of approximating distributions is to assume independencies that may not be present in the true posterior. This means that variational algorithms are often easy to parallelize. However, by searching only within a restricted class of models we lose some of the expressiveness of the model, and will typically obtain less accurate results than MCMC methods that sample from the true posterior.



\subsection{Approximate parallel Gibbs sampling}
An approximate distributed Gibbs sampler for the HDP is described in \cite{Asuncion:Smyth:Welling:2008}. The basic sampler alternates distributed Gibbs steps with a global synchronization step. If we have $P$ processors, in the distributed Gibbs steps, each processor updates $1/P$ of the topic allocations. To sample the topic allocation for a given token, rather than use the current topic allocations of \emph{all} the other tokens, we use the current topic allocations for the tokens on the same processor, and for all other tokens we use the allocations after the last synchronization step. In the synchronization step, we amalgamate the topic counts. This can run into problems with topic alignment. In particular, there is no clear way to decide whether to merge a new topic on processor $p$ with a new topic on processor $p'$. An asynchronous version of the algorithm avoids the bottleneck of a global synchronization step.



